"Inconsistent Performance": Understanding Concerns of Real-World Users on Smart Mobile Health Applications Through Analyzing App Reviews

While smart mobile health apps that adapt to users' progressive individual needs are proliferating, many of them struggle to fulfill their promises due to an inferior user experience. Understanding the concerns of real-world users related to those apps, and their smart components in particular, could help advance the app design to attract and retain users. In this paper, we target this issue through a preliminary thematic analysis of 120 user reviews of six smart health apps. We found that accuracy, customizability, and convenience of data input are primary concerns raised in real-world user reviews. Many concerns on the smart components are related to the trust issue of the users towards the apps. However, several important aspects such as privacy and fairness were rarely discussed in the reviews. Overall, our study provides insights that can inspire further investigations to support the design of smart mobile health apps.

==> s_relatedwork.tex <==
\section{Related Work}
\subsection{Mobile Health Apps}
With the continuous surge of new applications, there have been multiple studies done on specific types of applications serving a particular health need or group of users. For example, Niess et al.~\cite{Niess2021} conducted an interview-based study to understand attitudes and practices related to fitness tracking apps in a global setting. They proposed design suggestions to help build more inclusive fitness tracking apps. Lau et al.~\cite{Lau2020} conducted a systematic review of publicly available apps for psychosocial wellness and stress management. They found that only a very small fraction of such apps are backed up with scientific evidence of their effectiveness. Kao et al.~\cite{kao2017} reviewed a wide range of mobile health apps and identified three major barriers to advancing the potential of mobile health apps, including (1) lack of regulatory oversight, (2) limited evidence-based literature, and (3) concerns of privacy and security. Despite these previous efforts, there has been little research done particularly on the overall landscape of user opinions on health applications with a smart component. As a large percentage of previous research covers a distinct set of applications with a particular health function. Those studies although very valuable in understanding the specific concerns of users dealing with a specialized sub-section of health apps run into the risk of being too focused on domain-specific problems and leave a gap for observing the more general themes shared within most smart health apps brought up by the users that can be improved by further generalized solutions. This study aims to fill this gap.

\subsection{Design with Smart Components}
Many studies have been conducted to understand and address the new challenges when designing systems and applications that involve smart components. For example, Dove et al.~\cite{Dove2017} examined the design practice for applications with machine learning (ML) techniques by conducting a survey with UX practitioners. They questioned whether or not these practitioners took the ML component into account during their design process and discussed what new research and curriculum can help make the ML parts a more integral design material. Amershi et al.~\cite{Amershi2019} leveraged the rich literature in the history of HCI research and proposed 18 general design guidelines concerning learnability, error recovery, and evolution of AI systems. Volkel et al.~\cite{Volkel2020} aimed to decipher the essence of what makes a user interface intelligent by using a bottom-up approach to review the meaning of intelligence in user interface design literature and proposed their own definition of intelligence in UI. Our study is informed by this body of literature to examine user concerns of smart health apps.

\subsection{App Review Analysis}
Previous studies have used app reviews as a proxy to understand users' concerns in various types of apps. Vasa et al.~\cite{Vasa2012} conducted quantitative analysis on a large number of apps on Apple App Store; they found that the reviews are generally short and that lower ratings were correlated with longer reviews.


Ghosh et al.~\cite{Ghosh2018} qualitatively analyzed reviews written by children for online safety apps that are focused on parental control; they found that children considered these apps invasive to their privacy and damaging parent-children relationships. Prakash et al.~\cite{Prakash2020} developed a framework describing factors influencing user adoption of mental health conversational agents through a qualitative analysis of user review of such systems. Phillips et al.~\cite{Phillips2021} used user reviews of commercially available video games to identify games that have potential therapeutic values. Our methods are inspired by these previous studies.


